DualFocus: Integrating Macro and Micro Perspectives in Multi-modal Large Language Models

We present DualFocus, a novel framework for integrating macro and micro perspectives within multi-modal large language models (MLLMs) to enhance vision-language task performance. Current MLLMs typically singularly focus on inputs at a predefined resolution, resulting in deficiencies in detailed questions involving local regions. We introduced a DualFocus mechanism where the model concentrates on the image from a macro perspective, responses to the question, and identifies suitable sub-regions to zoom in for subsequent micro perspective analysis. Via the integration of answers from both macro and micro perspectives, the model is adept at addressing tasks that encompass global, detailed, and combined considerations. To endows the DualFocus mechanism in MLLMs, we curated a tailored dataset derived from the Visual Genome (VG) and adapted it to align with the training regimen of DualFocus. Through comparative studies across different model sizes and benchmarks, we demonstrate DualFocus's superiority in balancing detailed examination with holistic insight, significantly reducing hallucination instances in MLLMs and improving their performance in various vision-language tasks.

==> sections/impact.tex <==
\section*{Impact Statements}
The advent of DualFocus, an innovative approach in multi-modal large language models (MLLMs), heralds significant implications for society, encompassing both beneficial and adverse facets. 

On the positive side, DualFocus is poised to enhance machine comprehension of visual and textual data, thereby broadening the horizons of applications in assistive technologies, education, and information retrieval. Specifically, its nuanced understanding could revolutionize how visually impaired individuals interact with digital content, enabling these technologies to provide more accurate and contextually relevant information. Furthermore, in educational settings, this advanced comprehension capability can facilitate personalized learning experiences, particularly in visually intensive subjects such as biology and geometry, by adapting content to cater to the learner's inquiry with precision.

On the negative side,
%the adoption of DualFocus raises concerns regarding the amplification of existing societal disparities. 
% The enhanced capability of MLLMs could exacerbate digital divides if access to such advanced technologies remains unevenly distributed. Moreover, 
The potential for misuse in surveillance and data privacy cannot be overlooked. The ability of DualFocus models to interpret visual data with granular detail might pave the way for intrusive surveillance practices, risking individuals' privacy and autonomy.

In summary, while DualFocus promises to unlock new frontiers in human-computer interaction, echoing the dual nature of technological progress, it necessitates rigorous ethical scrutiny and equitable access strategies to ensure its benefits are universally accessible, thereby mitigating its societal risks.
